Port Protocols for Deadlock-Freedom of Component Systems

In component-based development, approaches for property verification exist that avoid building the global system behavior of the component model. Typically, these approaches rely on the analysis of the local behavior of fixed sized subsystems of components. In our approach, we want to avoid not only the analysis of the global behavior but also of the local behaviors of the components. Instead, we consider very small parts of the local behaviors called port protocols that suffice to verify properties.

==> eptcsdata.tex <==
\providecommand{\firstpage}{7}
\providecommand{\publicationstatus}{Bliudze, Bruni, Grohmann, Silva (Eds.):\\Third Interaction and Concurrency Experience (ICE 2010)\\
EPTCS 38, 2010, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.38.3}{10.4204/EPTCS.38.3}}
\pdfoutput=1

